Are NeRFs ready for autonomous driving? Towards closing the real-to-simulation gap

Neural Radiance Fields (NeRFs) have emerged as promising tools for advancing autonomous driving (AD) research, offering scalable closed-loop simulation and data augmentation capabilities. However, to trust the results achieved in simulation, one needs to ensure that AD systems perceive real and rendered data in the same way. Although the performance of rendering methods is increasing, many scenarios will remain inherently challenging to reconstruct faithfully. To this end, we propose a novel perspective for addressing the real-to-simulated data gap. Rather than solely focusing on improving rendering fidelity, we explore simple yet effective methods to enhance perception model robustness to NeRF artifacts without compromising performance on real data. Moreover, we conduct the first large-scale investigation into the real-to-simulated data gap in an AD setting using a state-of-the-art neural rendering technique. Specifically, we evaluate object detectors and an online mapping model on real and simulated data, and study the effects of different fine-tuning strategies.Our results show notable improvements in model robustness to simulated data, even improving real-world performance in some cases. Last, we delve into the correlation between the real-to-simulated gap and image reconstruction metrics, identifying FID and LPIPS as strong indicators. See https://research.zenseact.com/publications/closing-real2sim-gap for our project page.

==> sec/object_detection/bevformer.tex <==
% ----------------------- PETR -----------------------
\iffalse

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    BEVF-S given & 37.0 & 47.9 \\ 
    BEVF-S retrained & 39.3 & 49.8 \\
    BEVF-S w/ aug & 38.6 & 48.5 \\
    \midrule
    BEVF-S ft from given ckpt & 38.6 & 49.0 \\
    BEVF-S ft from given ckpt w/ aug & 38.6 & 48.5 \\
    BEVF-S ft from our ckpt & 39.1 & 49.6 \\
    BEVF-S ft from our ckpt w/ aug & 38.7 & 49.0 \\
    \bottomrule
    \end{tabular}
    \caption{BEVFormer performance on real validation data (150 scenes).}
    \label{tab:bevformer_real_val}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    BEVF-S given & 36.8 & 47.2 \\ 
    BEVF-S retrained & 38.8 & 49.2 \\
    BEVF-S w/ aug & 38.5 & 48.5 \\
    \midrule
    BEVF-S ft from given ckpt & 38.4 & 48.5 \\
    BEVF-S ft from given ckpt w/ aug & 38.5 & 48.1 \\
    BEVF-S ft from our ckpt & 38.7 & 49.1 \\
    BEVF-S ft from our ckpt w/ aug & 38.5 & 48.6 \\
    \bottomrule
    \end{tabular}
    \caption{BEVFormer performance on real validation data, clear weather subset.}
    \label{tab:bevformer_real_val_clear}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    BEVF-S given & 28.0 & 41.8 \\ 
    BEVF-S retrained & 29.5 & 43.6 \\
    BEVF-S w/ aug & 31.6 & 44.4 \\
    \midrule
    BEVF-S ft from given ckpt & 29.0 & 42.9 \\
    BEVF-S ft from given ckpt w/ aug & 30.6 & 43.6 \\
    BEVF-S ft from our ckpt & 29.6 & 43.9 \\
    BEVF-S ft from our ckpt w/ aug & 30.7 & 44.1 \\
    \bottomrule
    \end{tabular}
    \caption{BEVFormer performance on NeRF validation data, clear weather subset.}
    \label{tab:bevformer_nerf_val_clear}
\end{table}

\fi

\begin{table*}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $36.8$ & $47.2$ \\ 
                          & Yes         & None          &  2e-5     & $38.4$ & $48.5$ \\ 
                          & Yes         & Algorithmic   &  4e-5     & $38.9$ & $48.6$ \\ 
                          & Yes         & Algorithmic - opt   &  4e-5     & $38.2$ & $48.4$ \\ 
                          & Yes         & NeRF          &  4e-5     & $38.5$ & $48.3$ \\ 
                          & Yes         & Pix2Pix       &  4e-5     & $36.9$ & $47.2$ \\ 
                          & Yes         & Pix2Pix       &  4e-5, p=0.5 & $37.6$  & $47.7$ \\
                          \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $28.0$ & $41.8$ \\ 
                          & Yes         & None          &   2e-5        & $29.1$ & $42.7$ \\ 
                          & Yes         & Algorithmic   &   4e-5        & $31.0$ & $44.0$ \\ 
                          & Yes         & Algorithmic - opt  &   4e-5        & $29.5$ & $43.3$ \\ 
                          & Yes         & NeRF          &   4e-5        & $31.7$ & $44.5$ \\ 
                          & Yes         & Pix2Pix       &   4e-5        & $32.8$ & $44.8$ \\ 
                          & Yes         & Pix2Pix       &   4e-5, p=0.5 & $33.0$ & $44.9$ \\
    \bottomrule 
    \end{tabular}%}
    \caption{Various augmentation methods to close the real to simulation performance gap for BEVFormer.}
    \label{tab:fcos3d-real2sim-gap}
\end{table*}

==> sec/object_detection/collected_results.tex <==
\begin{table*}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $36.8$ & $47.2$ \\ 
                          & Yes         & None          &  2e-5     & $38.4$ & $48.5$ \\ 
                          & Yes         & Algorithmic   &  4e-5     & $38.9$ & $48.6$ \\ 
                          & Yes         & Algorithmic - opt   &  4e-5     & $38.2$ & $48.4$ \\ 
                          & Yes         & NeRF          &  4e-5     & $38.5$ & $48.3$ \\ 
                          & Yes         & Pix2Pix       &  4e-5     & $36.9$ & $47.2$ \\ 
                          & Yes         & Pix2Pix       &  4e-5, p=0.5 & $37.5$  & $48.1$ \\
                          \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $28.0$ & $41.8$ \\ 
                          & Yes         & None          &   2e-5        & $29.1$ & $42.7$ \\ 
                          & Yes         & Algorithmic   &   4e-5        & $31.0$ & $44.0$ \\ 
                          & Yes         & Algorithmic - opt  &   4e-5        & $29.5$ & $43.3$ \\ 
                          & Yes         & NeRF          &   4e-5        & $31.7$ & $44.5$ \\ 
                          & Yes         & Pix2Pix       &   4e-5        & $32.8$ & $44.8$ \\ 
                          & Yes         & Pix2Pix       &   4e-5, p=0.5 & $33.0$ & $44.9$ \\
    \bottomrule 
    \end{tabular}%}
    \caption{Various augmentation methods to close the real to simulation performance gap for BEVFormer.}
    \label{tab:fcos3d-real2sim-gap}
\end{table*}

\begin{table}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $32.2$ & $39.7$ \\ 
                          & Yes         & None          & $lr=2e-6$ & $32.2$ & $39.8$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $32.5$ & $40.0$ \\ 
                          & Yes         & NeRF          & $lr=1e-4$ & $31.2$ & $38.6$ \\ 
                          & Yes         & Pix2Pix       & $lr=1e-4$ & $32.5$ & $39.8$ \\ \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $13.6$ & $28.8$ \\ 
                          & Yes         & None          & $lr=2e-6$ & $13.5$ & $28.8$ \\ 
                          & Yes         & Algorithmic   & $lr=1e-5$ & $13.5$ & $28.9$ \\ 
                          & Yes         & NeRF          & $lr=1e-4$ & $23.5$ & $33.6$ \\ 
                          & Yes         & Pix2Pix       & $lr=1e-4$ & $24.5$ & $34.3$ \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Various augmentation methods to close the real to simulation performance gap for FCOS3D.}
    \label{tab:fcos3d-real2sim-gap}
\end{table}

\begin{table}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $38.3$ & $43.2$ \\ 
                          & Yes         & None          & $lr=1e-8$ & $38.6$ & $43.1$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $34.0$ & $38.9$ \\ 
                          & Yes         & NeRF          & $lr=2e-5$ & $35.1$ & $40.0$ \\ 
                          & Yes         & Pix2Pix       & $lr=2e-5$ & $31.4$ & $37.2$ \\ \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $18.8$ & $30.5$ \\ 
                          & Yes         & None          & $lr=1e-8$ & $20.2$ & $31.6$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $20.4$ & $30.0$ \\ 
                          & Yes         & NeRF          & $lr=2e-5$ & $29.3$ & $37.3$ \\ 
                          & Yes         & Pix2Pix       & $lr=2e-5$ & $26.1$ & $35.1$ \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Various augmentation methods to close the real to simulation performance gap for PETR.}
    \label{tab:petr-real2sim-gap}
\end{table}

\begin{table}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $38.3$ & $43.2$ \\ 
                          & Yes         & None          & $lr=1e-8$ & $38.6$ & $43.1$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $34.0$ & $38.9$ \\ 
                          & Yes         & NeRF          & $lr=2e-5$ & $35.1$ & $40.0$ \\ 
                          & Yes         & Pix2Pix       & $lr=2e-5$ & $31.4$ & $37.2$ \\ \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $18.8$ & $30.5$ \\ 
                          & Yes         & None          & $lr=1e-8$ & $20.2$ & $31.6$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $20.4$ & $30.0$ \\ 
                          & Yes         & NeRF          & $lr=2e-5$ & $29.3$ & $37.3$ \\ 
                          & Yes         & Pix2Pix       & $lr=2e-5$ & $26.1$ & $35.1$ \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Collected results.}
    \label{tab:collected-results}
\end{table}

==> sec/object_detection/fcos3d.tex <==
% ----------------------- FCOS3D -----------------------
\iffalse
\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    %\toprule
    Method & mAP & NDS \\ \midrule
    FCOS3D given &  &  \\ 
    %\midrule
    %\bottomrule
    \end{tabular}
    \caption{FCOS3D performance on real validation data (150 scenes).}
    \label{tab:FCOS3D_real_val}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    FCOS3D given & 32.2 & 39.7 \\ 
    \midrule
    FCOS3D ft (lr 2e-6) from given ckpt & 32.2 & 39.8 \\
    FCOS3D ft (lr 1e-5) from given ckpt w/ aug & 32.5 & 40.0 \\
    FCOS3D ft (lr 1e-4) from given ckpt w/ nerf (p=1) & 31.2 & 38.6 \\
    FCOS3D ft (lr 1e-4) from given ckpt w/ pix2pix (p=1) & 32.5 & 39.8 \\
    \bottomrule
    \end{tabular}
    \caption{FCOS3D performance on real validation data, clear weather subset.}
    \label{tab:FCOS3D_real_val_clear}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    FCOS3D given & 13.6 & 28.8 \\
    \midrule
    FCOS3D ft from given ckpt &  &  \\
    FCOS3D ft (lr 1e-5) from given ckpt w/ aug & 13.5 & 28.9 \\
    FCOS3D ft (lr 1e-4) from given ckpt w/ nerf (p=1) & 23.5 & 33.6 \\
    FCOS3D ft (lr 1e-4) from given ckpt w/ pix2pix (p=1) & 24.5 & 34.3 \\
    \bottomrule
    \end{tabular}
    \caption{FCOS3D performance on NeRF validation data, clear weather subset.}
    \label{tab:FCOS3D_nerf_val_clear}
\end{table}
 
\begin{table}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $32.2$ & $39.7$ \\ 
                          & Yes         & None          & $lr=2e-6$ & $32.2$ & $39.8$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $32.5$ & $40.0$ \\ 
                          & Yes         & NeRF          & $lr=1e-4$ & $31.2$ & $38.6$ \\ 
                          & Yes         & Pix2Pix       & $lr=1e-4$ & $32.5$ & $39.8$ \\ \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $13.6$ & $28.8$ \\ 
                          & Yes         & None          & $lr=2e-6$ & $13.5$ & $28.8$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $13.5$ & $28.9$ \\ 
                          & Yes         & NeRF          & $lr=1e-4$ & $23.5$ & $33.6$ \\ 
                          & Yes         & Pix2Pix       & $lr=1e-4$ & $24.5$ & $34.3$ \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Various augmentation methods to close the real to simulation performance gap for FCOS3D.}
    \label{tab:fcos3d-real2sim-gap}
\end{table}

\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c c c c c c c c c c}
    \hline 
    \toprule 
     & Augmentation & Shift         & Comment   & mAP    & NDS    & DA mAP & DA NDS  \\ \midrule  
     & Pix2Pix      & $-2$m         & $lr=1e-4$ & $17.4$ & $29.0$ & $11.5$ & $47.0$ \\
     & Pix2Pix      & $-1$m         & $lr=1e-4$ & $20.1$ & $30.3$ & $20.1$ & $54.4$ \\
     & Pix2Pix      & $0$m          & $lr=1e-4$ & $23.3$ & $33.1$ & $33.8$ & $59.7$ \\
     & Pix2Pix      & $0$m (real)   & $lr=1e-4$ & $30.9$ & $38.4$ & $-$    & $-$ \\
     & Pix2Pix      & $1$m          & $lr=1e-4$ & $19.6$ & $30.7$ & $15.5$ & $52.1$ \\
     & Pix2Pix      & $2$m          & $lr=1e-4$ & $15.6$ & $27.6$ & $10.0$ & $48.8$ \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Lane shift scores for FCOS3D. Detection agreement scores are aggregated per scene and averaged across all scenes.}
    \label{tab:fcos3d-lane-shift}
\end{table}
\fi
\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c c c c c c c}
    \hline 
    \toprule 
    \multirow{2}{*}{Probability of swap} & \multirow{2}{*}{Comment}  & \multicolumn{2}{c}{Sim}   & \multicolumn{2}{c}{Real} \\          
                                         &                           & mAP        & NDS          & mAP        & NDS         \\ \midrule  
     $p=0.1$                             & $lr=1e-4$                 & $18.0$     & $30.9$       & $30.9$     & $38.4$ \\
     $p=0.3$                             & $lr=1e-4$                 & $19.3$     & $31.8$       & $32.3$     & $39.4$ \\
     $p=0.5$                             & $lr=1e-4$                 & $20.3$     & $32.2$       & $32.4$     & $39.5$ \\
     $p=0.7$                             & $lr=1e-4$                 & $17.8$     & $30.3$       & $28.8$     & $37.3$ \\
     $p=1.0$                             & $lr=1e-4$                 & $24.5$     & $34.3$       & $32.5$     & $39.8$ \\
    \bottomrule 
    \end{tabular}%}
    \caption{FCOS3D fine-tuned with different probability of swapping the data sample with a pix2pix-image.}
    \label{tab:fcos3d-pix2pix-sweep}
\end{table}

==> sec/object_detection/petr.tex <==
% ----------------------- PETR -----------------------
\iffalse
\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    %\toprule
    Method & mAP & NDS \\ \midrule
    PETR given &  &  \\ 
    %\midrule
    %\bottomrule
    \end{tabular}
    \caption{PETR performance on real validation data (150 scenes).}
    \label{tab:PETR_real_val}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    PETR given & 38.3 & 43.2 \\ 
    \midrule
    PETR ft (lr 2e-6) from given ckpt &  &  \\
    PETR ft (lr 1e-5) from given ckpt w/ aug &  &  \\
    \bottomrule
    \end{tabular}
    \caption{PETR performance on real validation data, clear weather subset.}
    \label{tab:PETR_real_val_clear}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
    Method & mAP & NDS \\ \midrule
    PETR given & 18.8 & 30.5 \\
    \midrule
    PETR ft from given ckpt &  &  \\
    PETR ft (lr 1e-5) from given ckpt w/ aug &  &  \\
    PETR ft (lr 1e-4) from given ckpt w/ nerf (p=1) &  &  \\
    PETR ft (lr 1e-4) from given ckpt w/ pix2pix (p=1) &  &  \\
    \bottomrule
    \end{tabular}
    \caption{PETR performance on NeRF validation data, clear weather subset.}
    \label{tab:PETR_nerf_val_clear}
\end{table}

\begin{table}[t]
    \small
    \centering
    %\setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c c c c c}
    \hline 
    \toprule 
    Data                  & Finetuning  & Augmentation  & Comment   & mAP    & NDS \\ \midrule  
    \multirow{5}{*}{Real} & No          & None          &           & $38.3$ & $43.2$ \\ 
                          & Yes         & None          & $lr=1e-8$ & $38.6$ & $43.1$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $34.0$ & $38.9$ \\ 
                          & Yes         & NeRF          & $lr=2e-5$ & $35.1$ & $40.0$ \\ 
                          & Yes         & Pix2Pix       & $lr=2e-5$ & $31.4$ & $37.2$ \\ \midrule
    \multirow{5}{*}{Sim } & No          & None          &           & $18.8$ & $30.5$ \\ 
                          & Yes         & None          & $lr=1e-8$ & $20.2$ & $31.6$ \\ 
                          & Yes         & Algorithmic   & $lr=2e-5$ & $20.4$ & $30.0$ \\ 
                          & Yes         & NeRF          & $lr=2e-5$ & $29.3$ & $37.3$ \\ 
                          & Yes         & Pix2Pix       & $lr=2e-5$ & $26.1$ & $35.1$ \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Various augmentation methods to close the real to simulation performance gap for PETR.}
    \label{tab:petr-real2sim-gap}
\end{table}

\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c c c c c c c c}
    \hline 
    \toprule 
     & Augmentation & Shift         & Comment   & mAP    & NDS    & DA mAP  & DA NDS    \\ \midrule  
     & NeRF         & $-2$m         & $lr=2e-5$ & $22.5$ & $31.3$ & $33.9$  & $52.8$ \\
     & NeRF         & $-1$m         & $lr=2e-5$ & $25.4$ & $33.2$ & $42.0$  & $58.1$ \\
     & NeRF         & $0$m          & $lr=2e-5$ & $27.5$ & $35.0$ & $47.9$  & $62.7$ \\
     & NeRF         & $0$m (real)   & $lr=2e-5$ & $35.5$ & $40.1$ & $-$     & $-$ \\
     & NeRF         & $1$m          & $lr=2e-5$ & $25.0$ & $33.3$ & $41.7$  & $57.3$ \\
     & NeRF         & $2$m          & $lr=2e-5$ & $21.9$ & $30.8$ & $34.7$  & $52.1$ \\
    \bottomrule 
    \end{tabular}%}
    \caption{Lane shift scores for PETR. Detection agreement scores are aggregated per scene and averaged across all scenes.}
    \label{tab:petr-lane-shift}
\end{table}
\fi

\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c c c c c}
    \hline 
    \toprule 
    \multirow{2}{*}{Probability of swap} & \multirow{2}{*}{Comment}  & \multicolumn{2}{c}{Sim}   & \multicolumn{2}{c}{Real} \\          
                                         &                           & mAP        & NDS          & mAP        & NDS         \\ \midrule  
    $p=0.1$                              & $lr=2e-5$                 & $22.0$     & $31.6$       & $36.7$     & $41.2$      \\
    $p=0.3$                              & $lr=2e-5$                 & $23.6$     & $33.7$       & $36.3$     & $41.4$      \\
    $p=0.5$                              & $lr=2e-5$                 & $25.6$     & $34.9$       & $36.0$     & $41.2$      \\
    $p=0.7$                              & $lr=2e-5$                 & $26.9$     & $35.5$       & $35.6$     & $40.9$      \\
    $p=1.0$                              & $lr=2e-5$                 & $26.1$     & $35.1$       & $31.4$     & $37.2$      \\
    \bottomrule 
    \end{tabular}%}
    \caption{PETR fine-tuned with different probability of swapping the data sample with a pix2pix-image.}
    \label{tab:petr-pix2pix-sweep}
\end{table}

\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c c c c c}
    \hline 
    \toprule 
    \multirow{2}{*}{Probability of swap} & \multirow{2}{*}{Comment}  & \multicolumn{2}{c}{Sim}   & \multicolumn{2}{c}{Real} \\          
                                         &                           & mAP        & NDS          & mAP        & NDS         \\ \midrule
     $p=0.1$                             & $lr=2e-5$                 & $25.7$     & $34.6$       & $36.5$     & $41.3$ \\
     $p=0.3$                             & $lr=2e-5$                 & $27.9$     & $36.1$       & $36.8$     & $41.6$ \\
     $p=0.5$                             & $lr=2e-5$                 & $28.4$     & $36.5$       & $36.9$     & $41.6$ \\
     $p=0.7$                             & $lr=2e-5$                 & $28.8$     & $36.6$       & $36.7$     & $41.6$ \\
     $p=1.0$                             & $lr=2e-5$                 & $29.3$     & $37.3$       & $35.1$     & $40.0$ \\
    \bottomrule 
    \end{tabular}%}
    \caption{PETR fine-tuned with different probability of swapping the data sample with a NeRF-image.}
    \label{tab:petr-nerf-sweep}
\end{table}

==> sec/online_mapping/maptrv2.tex <==

\begin{table*}[t]
    \small
    \centering
    \caption{Real2sim results for the online mapping method on both data splits, fine-tuned with different strategies. "Sim" indicates that the model was evaluated on rendered data from NeuRAD.}
    \setlength\extrarowheight{-5pt}
    \setlength{\tabcolsep}{3pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{c c @{\hskip 15pt} cccc @{\hskip 15pt} c @{\hskip 15pt}| @{\hskip 15pt} cccc @{\hskip 15pt} c }
    \hline 
    \toprule 
    \multirow{3}{*}{\begin{tabular}{c}Fine-tuning \\ Method\end{tabular}} & \multirow{3}{*}{\begin{tabular}{c}Evaluation \\ Data\end{tabular}} & \multicolumn{5}{c}{Original} & \multicolumn{5}{c}{Geographically Disjoint} \\  
    & &         \multicolumn{4}{c}{mAP} & DA & \multicolumn{4}{c}{mAP} &  DA \\ 
    &                                                     & Divider & Boundary & Crossing & Mean & & Divider & Boundary & Crossing & Mean  &         \\ \midrule
    \multirow{3}{*}{Real data only}         & Real        & $64.3$ & $65.6$ & $63.7$ & $64.5$ & 100.0 & $23.1$ & $36.5$ & $20.3$ & $26.6$ & 100.0 \\ 
                                  & Sim                   & $57.2$ & $56.5$ & $48.2$ & $54.0$ & 71.8  & $20.2$ & $32.4$ & $16.9$ & $23.2$ & 67.1  \\ 
                                  & Gap (\%)              & $10.7$ & $13.9$ & $24.3$ & $16.3$ & 28.2  & $12.6$ & $11.2$ & $16.7$ & $12.8$ & 32.9  \\ \midrule
    \multirow{3}{*}{\begin{tabular}{c}Image \\ augmentations\end{tabular}}  & Real                  & $64.9$ & $66.4$ & $64.0$ & $65.1$ & 100.0 & $23.4$ & $37.1$ & $19.0$ & $26.5$ & 100.0  \\
                                  & Sim                   & $58.3$ & $57.8$ & $49.6$ & $55.2$ & 72.3  & $21.2$ & $33.7$ & $16.5$ & $23.8$ & 70.1  \\ 
                                  & Gap (\%)              & $ 9.3$ & $11.9$ & $22.1$ & $14.4$ & 27.7  & $ 8.2$ & $ 7.7$ & $18.7$ & $10.5$ & 29.9  \\  \midrule
    \multirow{3}{*}{NeRF}         & Real                  & $64.7$ & $65.9$ & $64.1$ & $64.9$ & 100.0 & $23.8$ & $37.2$ & $19.8$ & $26.9$ & 100.0  \\
                                  & Sim                   & $58.9$ & $58.2$ & $50.8$ & $56.0$ & 74.5  & $22.0$ & $34.6$ & $17.1$ & $24.6$ & 70.5  \\ 
                                  & Gap (\%)              & $ 8.4$ & $11.3$ & $20.3$ & $13.2$ & 25.5  & $ 4.8$ & $ 5.2$ & $15.8$ & $ 7.5$ & 29.5  \\  \midrule
    \multirow{3}{*}{Image-to-image}      & Real           & $62.2$ & $64.7$ & $62.6$ & $62.5$ & 100.0 & $21.3$ & $36.3$ & $18.0$ & $25.2$ & 100.0 \\ 
                                  & Sim                   & $60.0$ & $58.9$ & $51.6$ & $56.8$ & 74.8  & $20.6$ & $34.9$ & $17.5$ & $24.3$ & 73.9  \\ 
                                  & Gap (\%)              & $ 6.7$ & $10.2$ & $19.2$ & $11.9$ & 25.2  & $10.8$ & $ 4.4$ & $13.8$ & $ 8.3$ & 26.1  \\  

    \bottomrule 
    \end{tabular}%}
    \label{tab:real2sim-results-OM}
    \vspace{-15pt}
\end{table*}

%\begin{table}[t]
%    \small
%    \centering
%    \renewcommand{\arraystretch}{0.75}
%    \setlength{\tabcolsep}{1pt} % Default value: 6pt
%    %\scalebox{0.8}{%
%    \begin{tabular}{l c c cc cc cc cc c}
%    \hline 
%    \toprule 
%    & Data & Finetune & Augmentation & Divider  & Boundary & Crossing & Mean  \\ \midrule  
%    \multirow{6}{*}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Original}}}} 
%    &\multirow{5}{*}{Real} & No       & None                & $64.1$ & $65.9$ & $63.6$ & $64.5$ \\ 
%    &                      & Yes      & None                & $64.3$ & $65.6$ & $63.7$ & $64.5$ \\ 
%    &                      & Yes      & Algorithmic         & $64.9$ & $66.4$ & $64.0$ & $65.1$ \\ 
%    &                      & Yes      & NeRF                & $64.7$ & $65.9$ & $64.1$ & $64.9$ \\ 
%    &                      & Yes      & Pix2Pix             & $62.2$ & $64.7$ & $62.6$ & $62.5$ \\ \cmidrule{3-8} 
%    &\multirow{5}{*}{Sim } & No       & None                & $56.9$ & $56.6$ & $48.2$ & $53.9$ \\ 
%    &                      & Yes      & None                & $57.2$ & $56.5$ & $48.2$ & $54.0$ \\ 
%    &                      & Yes      & Algorithmic         & $58.3$ & $57.8$ & $49.6$ & $55.2$ \\ 
%    &                      & Yes      & NeRF                & $57.6$ & $56.5$ & $49.2$ & $54.4$ \\ 
%    &                      & Yes      & Pix2Pix             & $60.0$ & $58.9$ & $51.6$ & $56.8$ \\ \cmidrule{2-8} 
%    \multirow{6}{*}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Geographical}}}} 
%    &\multirow{5}{*}{Real} & No       & None                & $23.3$ & $36.7$ & $19.7$ & $26.6$  \\ 
%    &                      & Yes      & None                & $23.1$ & $36.5$ & $20.3$ & $26.6$  \\ 
%    &                      & Yes      & Algorithmic         & $23.4$ & $37.1$ & $19.0$ & $26.5$  \\ 
%    &                      & Yes      & NeRF                & $23.8$ & $37.2$ & $19.8$ & $26.9$  \\ 
%    &                      & Yes      & Pix2Pix             & $21.3$ & $36.3$ & $18.0$ & $25.2$  \\ \cmidrule{3-8} 
%    &\multirow{5}{*}{Sim } & No       & None                & $20.5$ & $32.5$ & $16.4$ & $23.2$  \\ 
%    &                      & Yes      & None                & $20.2$ & $32.4$ & $16.9$ & $23.2$  \\ 
%    &                      & Yes      & Algorithmic         & $21.2$ & $33.7$ & $16.5$ & $23.8$  \\ 
%    &                      & Yes      & NeRF                & $22.0$ & $34.6$ & $17.1$ & $24.6$  \\ 
%    &                      & Yes      & Pix2Pix             & $20.6$ & $34.9$ & $17.5$ & $24.3$  \\ 
%    \bottomrule 
%    \end{tabular}%}
%    \caption{Various augmentation methods to close the real to simulation performance gap for the online mapping method MapTRv2 on the Original and Geographical splits }
%    \label{tab:maptrv2-sim2real-gap}
%\end{table}

==> sec/online_mapping/maptrv2_agreement.tex <==
\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c cc cc cc cc c}
    \hline 
    \toprule 
    & Finetuning & Augmentation & Divider  & Boundary & Crossing & Mean & Diff \\ \midrule  
    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Original}}}} 
    & No       & None                & $73.2$ & $76.8$ & $65.3$ & $71.8$ & Ref  \\ 
    & Yes      & None                & $73.2$ & $76.9$ & $65.3$ & $71.8$ & $+0.0$  \\ 
    & Yes      & Algorithmic         & $72.8$ & $77.4$ & $66.8$ & $72.3$ & $+0.6$  \\ 
    & Yes      & NeRF                & $75.5$ & $79.6$ & $68.3$ & $74.5$ & $+2.7$  \\ 
    & Yes      & Pix2Pix             & $76.2$ & $79.7$ & $68.6$ & $74.8$ & $+3.1$  \\ \cmidrule{2-8} 
    \multirow{3}{*}{\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Geogr.}}}} 
    & No       & None                & $60.9$ & $72.6$ & $69.4$ & $67.6$ & Ref  \\ 
    & Yes      & None                & $60.0$ & $73.3$ & $68.2$ & $67.1$ & $-0.5$ \\ 
    & Yes      & Algorithmic         & $62.6$ & $75.4$ & $72.4$ & $70.1$ & $+2.5$  \\ 
    & Yes      & NeRF                & $64.1$ & $77.7$ & $69.8$ & $70.5$ & $+2.9$ \\ 
    & Yes      & Pix2Pix             & $67.0$ & $80.8$ & $73.9$ & $73.9$ & $+6.3$  \\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Agreement scores for the different training methods on MapTRv2}
    \label{tab:maptrv2-sim2real-agreement}
\end{table}

==> sec/online_mapping/maptrv2_lane_shift.tex <==
%\begin{table}
%    \small
%    \centering
%    \renewcommand{\arraystretch}{0.8}
%    \setlength{\tabcolsep}{2pt} % Default value: 6pt
%    %\scalebox{0.8}{%
%    \begin{tabular}{l c cc cc cc cc c c c}
%    \hline 
%    \toprule 
%     & Augmentation & Real  & Sim & $-2$m & $-1$m & $+1$m & $+2$m & $\pm 1$m & $\pm 2$m \\ \midrule  
%    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Original}}}} 
%          & None                   & $62.5$ & $55.4$ & $47.4$ & $45.9$ & $36.3$ & $35.2$ & $46.7$ & $35.8$  \\ 
%          & Algorithmic            & $62.2$ & $55.3$ & $49.2$ & $47.9$ & $37.1$ & $36.2$ & $48.6$ & $36.7$ \\ 
%          & NeRF                   & $63.0$ & $57.4$ & $50.7$ & $49.1$ & $39.1$ & $37.8$ & $49.9$ & $38.5$ \\ 
%          & Pix2Pix                & $60.6$ & $59.2$ & $51.5$ & $51.5$ & $39.0$ & $40.2$ & $51.5$ & $39.6$ \\  \cmidrule{2-10} 
%    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Geogr.}}}} 
%          & None                & $29.2$ & $25.1$ & $20.6$ & $19.0$ & $17.0$ & $14.1$ & $19.8$ & $15.6$\\ 
%          & Algorithmic         & $29.3$ & $26.1$ & $21.4$ & $19.8$ & $17.9$ & $14.8$ & $20.6$ & $16.3$\\ 
%          & NeRF                & $29.5$ & $26.5$ & $23.2$ & $20.8$ & $17.9$ & $15.1$ & $22.0$ & $16.5$\\ 
%          & Pix2Pix             & $26.9$ & $25.7$ & $23.9$ & $18.5$ & $21.8$ & $16.6$ & $21.2$ & $19.2$\\ 
%    \bottomrule 
%    \end{tabular}%}
%    \caption{Lane shift scores for the different training methods on MapTRv2}
%    \label{tab:maptrv2-lane-shift}
%\end{table}


\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.75}
    \setlength{\tabcolsep}{1pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c cc cc c c c}
    \hline 
    \toprule 
     & Augmentation & Real  & Sim & $\pm 1$m & $\pm 2$m \\ \midrule  
    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Original}}}} 
          & None                   & $62.5$ & $55.4$ & $46.7$ & $35.8$  \\ 
          & Algorithmic            & $62.2$ & $55.3$ & $48.6$ & $36.7$ \\ 
          & NeRF                   & $63.0$ & $57.4$ & $49.9$ & $38.5$ \\ 
          & Pix2Pix                & $60.6$ & $59.2$ & $51.5$ & $39.6$ \\  \cmidrule{2-6} 
    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Geogr.}}}} 
          & None                & $29.2$ & $25.1$ & $19.8$ & $15.6$\\ 
          & Algorithmic         & $29.3$ & $26.1$ & $20.6$ & $16.3$\\ 
          & NeRF                & $29.5$ & $26.5$ & $22.0$ & $16.5$\\ 
          & Pix2Pix             & $26.9$ & $25.7$ & $21.2$ & $19.2$\\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Lane shift scores for the different training methods on MapTRv2}
    \label{tab:maptrv2-lane-shift}
\end{table}

==> sec/online_mapping/maptrv2_rotation.tex <==
\begin{table}[t]
    \small
    \centering
    \renewcommand{\arraystretch}{0.75}
    \setlength{\tabcolsep}{2pt} % Default value: 6pt
    %\scalebox{0.8}{%
    \begin{tabular}{l c cc ccccc}
    \hline 
    \toprule 
     & Augmentation & Real  & Sim & $\pm 5^{\circ}$ & $\pm 15^{\circ}$ & $\pm 30^{\circ}$ & $\pm 90^{\circ}$ & $180^{\circ}$ \\ \midrule  
    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Original}}}} 
          & None                   & $64.5$ & $54.0$ & $49.4$ & $32.7$ & $17.4$ & $5.9$ & $17.4$ \\ 
          & Algorithmic            & $65.1$ & $55.2$ & $51.7$ & $34.4$ & $18.3$ & $6.5$ & $18.4$ \\ 
          & NeRF                   & $64.9$ & $54.4$ & $53.1$ & $35.3$ & $19.3$ & $6.8$ & $19.1$ \\ 
          & Pix2Pix                & $62.5$ & $56.8$ & $53.9$ & $35.4$ & $19.3$ & $6.4$ & $19.5$ \\  \cmidrule{2-9} 
    \multirow{2}{*}{\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Geogr.}}}} 
          & None                & $26.6$ & $23.2$ & $21.5$ & $16.1$ & $10.6$ & $5.0$ & $10.6$ \\ 
          & Algorithmic         & $26.5$ & $23.8$ & $21.9$ & $16.8$ & $11.2$ & $5.4$ & $11.4$ \\ 
          & NeRF                & $26.9$ & $24.6$ & $22.6$ & $17.3$ & $11.4$ & $5.2$ & $12.1$ \\ 
          & Pix2Pix             & $25.2$ & $24.3$ & $22.2$ & $17.4$ & $11.9$ & $5.8$ & $12.8$\\ 
    \bottomrule 
    \end{tabular}%}
    \caption{Rotation scores for the different training methods on MapTRv2}
    \label{tab:maptrv2-rotation}
\end{table}
